OptMark: A Toolkit for Benchmarking Query Optimizers

Query optimizers have long been considered as among the most complex components of a database engine, while the assessment of an optimizer's quality remains a challenging task. Indeed, existing performance benchmarks for database engines (like TPC benchmarks) produce a performance assessment of the query runtime system rather than its query optimizer. To address this challenge, this paper introduces OptMark, a toolkit for evaluating the quality of a query optimizer. OptMark is designed to offer a number of desirable properties. First, it decouples the quality of an optimizer from the quality of its underlying execution engine. Second it evaluates independently both the effectiveness of an optimizer (i.e., quality of the chosen plans) and its efficiency (i.e., optimization time). OptMark includes also a generic benchmarking toolkit that is minimum invasive to the DBMS that wishes to use it. Any DBMS can provide a system-specific implementation of a simple API that allows OptMark to run and generate benchmark scores for the specific system. This paper discusses the metrics we propose for evaluating an optimizer's quality, the benchmark's design and the toolkit's API and functionality. We have implemented OptMark on the open-source MySQL engine as well as two commercial database systems. Using these implementations we are able to assess the quality of the optimizers on these three systems based on the TPC-DS benchmark queries.

==> effectiveness.tex <==
\section{Optimization Effectiveness}\label{s_effectivenss}

- Our goal here is to evaluate  the quality of the plan picked by the optimizer. 

- This involves studying the quality of the chosen execution plan relative to the plans that the optimizer considered and designing metrics for quantifying this quality. 


- Describe our approach: Our approach identifies the best candidate execution plan that the optimizer could have considered for a given query and compare it with the final plan of a specific optimizer. 

- Describe our effectiveness metric: given a set of benchmark queries, our tool will do the following:
   (a) for each query will identify the best candidate query plan and record its execution time
   (b) it will execute the query plan picked by the optimizer and record its execution time
   (c) it calculate the "effectiveness" percentage as the \% of times the optimizer picked the actual best plan
   
-Challenges of this process: avoid exhaustive enumeration of candidate plans by pruning some plan while maintaining good quality plans in the candidate set (i.e., we don't want our pruning to eliminate the best plan). 

\subsection{JPEG-based plan elimination}

- Outline our approach and the motivation behind using JPEG

- Describe JPEG with Illustrative examples to demonstrate how JPEG works  

- Describe some of the ranking we used for JPEG and the motivation behind them

\subsection{Effectiveness API}

- Describe the API

- Give examples of the API on 1-2 engine



==> efficiency.tex <==

\section{Optimization Efficiency}\label{s_efficiency}
 
- Our goal is to evaluate how efficient in terms of time the optimization process is. Hence, we extensively studied the  optimization time of various optimizers and its relationship to a number of  statistical properties of the optimization process. We were able to identified a set of properties which demonstrate strong correlation with the optimization time and hence can be used to compare the efficiency of different optimizers. We refer to these properties as  \emph{efficiency indicators}.  In the next section we discuss these indicators and how their correlation to the optimization time. 

- We studied the optimization time of  TPC-DS queries and a number of database engines (SQL Server, PostgreSQL, MySQL and Oracle). Our study revealed strong correlation of the optimization with four properties of the optimization process: 

(discuss each indicator, briefly give the intuition of why it was found to be relevant to the optimization time)

(1) number of logical plans, 

(2) number of logical join plans

(3) number of physical plans and 

(4) number of physical join plans. 


- All these properties can be used as indicators of the optimization efficiency. 

-These indicators are easily extractable from all optimizer and they are independent of the underlying execution engine and optimization environment. 

\subsection{Efficiency API}

- One paragraph that says that the API here is straightforward and describe briefly how we did in  the 4 DBs we used. 



==> experiments.tex <==
\section{Experimental Results}\label{s_experiments}

\subsection{Experimental setup}

- which benchmarks we used

-which DBs engines we used 

-For each engines which data structures and we used and any extra processing we had to do on the data they provided 


\subsection{Effectiveness metrics}

- add linear regression numbers here, explain the results for each engine

- maybe add a few metrics (obvious choices)  that were not correlated and explain why we do not use them in the tool?
 
 \subsection{Efficiency metric}
 
 - show the results on the efficiency metric on the different machines
 
 - group them by number of join 
 
 - explain the results 





==> intro.tex <==
\section{Introduction}\label{s_intro}



==> toolkit3_2_2.tex <==
\subsubsection{Benchmarking Effectiveness}\label{s:effectivenessAlgo}
 
Next we describe OptMark's approach for assessing the effectiveness of an optimizer. Given a set of queries to execute the benchmark on and an implementation of the effectiveness API for the DBMS OptMark is running on, our toolkit generates a set of random sample physical plans against which the optimizer chosen plan is compared in plan runtime. The effectiveness benchmarking workflow for a single query is show in Figure~\ref{f:effectivenessworkflow}. OptMark focuses on three factors when generating the sample set: join ordering, join methods and table access methods.

As discussed in section 2.1.1, the size of the samples is determined by user-desired confidence level and margin of error. OptMark allows user to specify any two of confidence level, margin of error and time budget, and it will present the third one. For example, if the user wants to run OptMark for an hour and desires 95\% confidence level, OptMark will generate and run as many random plans as possible in an hour and compare each plan with optimizer's plan then report the performance factor with confidence level and margin of error. Suppose the given query involves $m$ joins, the plans with which the optimizer-chosen plan is compared are generated as follows:\\

 
\begin{figure}
\centering
\includegraphics[width=3.2in,angle=0]{figs/Optimizer-Effectiveness-Assessment2.pdf}
\caption{Effectiveness Benchmarking Workflow}

\label{f:effectivenessworkflow}
\end{figure}


 \begin{enumerate}
 \item Generate a random join ordering as discussed in section 2.1.2.
 \item Create a SQL query that enforces specified join ordering generated in step 1.
 \item For each of the $m$ joins in the join ordering, randomly select one physical join operation from all physical join operations returned by {\tt joinType()}. The enforced join orderings of step 2 and the choice of join operations in step 3 is enforced according to directives specified in {\tt joinHint()}.
 \item For every table in the query with an index on a predicate attribute, randomly select to use index by adding SQL directive specified by {\tt indexHint()} or use sequential scan.
 \item Repeat step 1 - 4 to generate a random plan until reach time budget specified by the user or the sample size determined by user desired confidence level and margin of error.
 \end{enumerate}
 
Once the benchmark is run, it returns the performance factor of that query. The process is applied for all queries in a given benchmarking workload and then performance factor and optimality frequency of the workload as defined in Section~\ref{s:effectiveness} is reported.
